Importance of negative sampling in weak label learning

Weak-label learning is a challenging task that requires learning from data "bags" containing positive and negative instances, but only the bag labels are known. The pool of negative instances is usually larger than positive instances, thus making selecting the most informative negative instance critical for performance. Such a selection strategy for negative instances from each bag is an open problem that has not been well studied for weak-label learning. In this paper, we study several sampling strategies that can measure the usefulness of negative instances for weak-label learning and select them accordingly. We test our method on CIFAR-10 and AudioSet datasets and show that it improves the weak-label classification performance and reduces the computational cost compared to random sampling methods. Our work reveals that negative instances are not all equally irrelevant, and selecting them wisely can benefit weak-label learning.

==> brain_dump.tex <==
% The importance of weakly-labeled learning stems from several factors:

% Cost-Efficiency
% Collecting perfectly labeled data can be expensive both in terms of time and resources. Weakly-labeled learning allows models to learn from data that is cheaper and quicker to collect.

% Scalability
% Weak labels often make it feasible to collect much larger datasets. Large datasets are essential for training sophisticated machine learning models, particularly deep learning models that have many parameters.

% Real-world Applicability
% In many real-world scenarios, perfect labeling is not possible. For example, in medical settings, it might be unrealistic to expect perfect diagnoses for training data. Weak labels reflect the kinds of data that are often available in practice.

% Human-in-the-loop
% Weak labels can often be generated with minimal human intervention, making it easier to integrate human expertise. For example, experts can provide "rules of thumb" that generate weak labels across a large dataset, which can then be refined through machine learning.

% Flexibility
% Weak labels can come in many forms: they could be noisy labels, partial labels, or even labels that come from multiple annotators with varying expertise. This flexibility makes weakly-labeled learning widely applicable across different domains and problems.

% Data Augmentation
% Weakly-labeled data can often serve as a useful supplement to small amounts of strongly-labeled data, effectively augmenting the dataset and improving the model's performance.

% Ethical Considerations
% In sensitive applications, weak labeling can offer a path to mitigate biases that may be present in hand-curated, strongly labeled datasets.

% Bootstrapping
% In many cases, models trained on weakly labeled data can be used to generate better labels for other datasets, or even for refining labels in the original dataset, in a bootstrapping process.

% Rapid Prototyping
% In cases where getting a model up and running quickly is more important than achieving the best possible performance, weak labels can expedite the development process.

% Weakly-labeled learning is particularly important for problems where data is abundant, but labels are scarce or expensive. It has found applications in a variety of fields, including natural language processing, computer vision, healthcare, and more.






% \textbf{\textit {Weak label learning}} has gained significant attention in recent research \cite{sun2010multi,shah2018closer,wang2020learning}. Contrary to traditional supervised learning, weak-label learning conduct multi-label training in a weakly-supervised way, which presents as an advantage in many tasks, e.g., audio classification \cite{shah2018closer}. In the weak label learning setting, samples have multiple ground-truth labels but only part of them are provided. 
% How to effectively train a model using these partially labeled samples usually becomes the focus in many studies.
%consist of noise and multiple instances, which jeopardize the performance of multi-label learning. 


% Our paper aims to find an approach to actively sample proper negative bags based on informativeness and diversity under a weak label setting. Our approach applies to various weak-label learning tasks, including image and audio classification. Through our experiments, we established an implicit relationship between the contribution, uncertainty, similarity, and diversity of negative bags. We could learn a better weak classifier with a reasonable label budget by sampling informative negative bags.


% In this research paper, we introduce a novel methodology designed to actively and intelligently sample "negative bags" in a weakly-supervised learning setting. This methodology is grounded in the principles of informativeness and diversity, aiming to maximize the utility of each sampled negative bag. Our framework is versatile, capable of enhancing performance across a range of weak-label learning applications, including but not limited to image and audio classification tasks.

% Through rigorous experimentation, we have uncovered a nuanced interplay among four key factors: the contribution, uncertainty, similarity, and diversity of negative bags. By strategically selecting negative bags that are both informative and diverse, our approach enables the construction of a more robust and efficient weak classifier. Importantly, this is achieved without an excessive labeling budget, streamlining the learning process and making it more cost-effective.

%
% Our proposal could be applied to general cases in different weak-label learning tasks like image or audio. Based on our experiment results, we could implicitly form the relationship between the contribution, uncertainty, similarity, and diversity of negative bags.

% In summary, the main contribution of this paper include:
% \begin{itemize}
% \item We introduce the definition of negative sampling for weak label learning to find informative negative bags and improve classification results.
% \item We demonstrate the applicability of the existing sampling strategy under weak label setting in 2 classification tasks: 1) Image Bag Classification and 2) Audio Classification. By sampling proper negative bags from the data pool, we could save data budget while maintaining a relatively good classification performance. 

%\item More specifically, whether negative data is similar to or different from the target object contributes more to the classification results and how to measure that;
%\item Can the data selection strategy (Negative Sampling) be modeled for different tasks using weak labels combined with negative sampling;
%% may remove this 
%\item To what proportion should the positive against negative instances enough to train a classifier?



%We look to address the following: how to choose a reasonable sampling strategy? The sampling strategy we designed should identify the most informative negative samples that can help learn the best classifier with a reasonable label budget, which is also the core problem in the active learning research field. That's why we introduce this topic in our project. Even though active learning aims to sample unlabeled data while only negative instances are our focus, the method will intrinsically select informative data samples that can improve the learning of the model and thus enhance the discriminative and predictive ability of the model. In other words, the active learning algorithm will only select the data samples that are closest to the actual decision boundary disregarding irrelevant data samples from consideration, which will hopefully give us guidance on how to choose our negative samples.

%In the future, this project has a profound meaning for guiding the industrial data labeling on how much data is needed, what kind of data is preferred, and what ratio of positive to negative samples is required for confident classification. 

% Many active learning-based sampling strategies have shown good performance in model training nowadays. Widely used Uncertainty-based strategies, e.g., entropy sampling and margin sampling, improve the prediction performance by selecting data samples that models mostly struggle with. 
% % In one way, these sampling strategies increase the capability of machines to answer hard questions; but in another way, they narrow down the models' view by a small diversity of data. 
% WKMeans\cite{zhdanov2019diverse} and BADGE sampling strategy\cite{ash2019deep} try to solve this problem by introducing more diversity. 
% % They use KMeans method to choose informative data samples as well as ones from far way, making it easier for model to see a variety of data samples. 
% Hard Negative sampling \cite{robinson2020contrastive} focuses on sampling data samples with high hardness in contrastive learning, clustering each class while pushing different classes far away.  However, most of the strategies above are conducted under strong label settings. Their capability and robustness in weak label learning required additional validation. 



% Data selection methods pick a subset of data that is most useful and informative for a given task. They help avoid overfitting by balancing data distribution and enhancing model's generalization ability by having diverse data samples. Models trained using weak labels utilize the presence or absence of an event over fine-grained annotation information. Current research on weak labels has studied sampling strategies for informative querying of data whereas the overall importance of selecting negatives in weak label learning remains under explored. In this paper, we study the selection of more informative negative samples, and the underlying principles to quantify the importance of the bag data. Our experiment results on CIFAR-10 and AudioSet demonstrate that an effective negative sampling strategy can improve classification performance over random sampling under weak label settings. 


% While data selection methods have proven indispensable in curating highly informative and balanced datasets for strongly-labeled learning, their efficacy in the realm of weak-label learning remains an open question—particularly concerning the largely unexplored space of negative instances. This paper addresses this critical gap by introducing a groundbreaking framework specifically designed to evaluate the utility of negative samples in weakly-labeled learning environments. Rooted in principled methodologies, our approach quantifies the importance of negative samples within a data "bag," thereby offering a targeted strategy for their selection. We conduct experiments on CIFAR-10 and AudioSet databases and demonstrate that an efficient negative sampling approach consistently outperforms random sampling techniques, particularly in the nuanced context of weak-label classification. These findings underscore a paradigm shift: the key to enhancing model performance and computational efficiency lies not only in the judicious selection of positive instances but also in the strategic inclusion of informative negative instances.


% Data selection methods aim to curate a subset of the most beneficial and informative data for specific tasks, enhancing a model's ability to generalize by ensuring a balanced and diverse dataset. These methods are instrumental in preventing overfitting due to diverse data samples. The diversity of the samples has been well studied in the context of strongly labeled learning. However, in the case of weak labels, existing research primarily focuses on how to effectively query or sample positive instances or events present in the data. In contrast, the large repository of negative events is underexplored. This paper delves into the importance of strategically selecting negative samples when working with weak labels. We introduce a framework for evaluating the utility of negative samples and propose underlying principles for quantifying their importance within a "bag" of data. We conduct experiments using each sampling strategy in the CIFAR-10 and AudioSet databases, Our results show that employing an intelligent negative sampling strategy outperforms random sampling, specifically in the context of weak label classification tasks. We find the proposed  sampling strategies always effective  This underscores the importance of not just selecting informative positive instances, but also informative negative instances, for improving model performance and speed.

% Models trained using weak labels utilize the presence or absence of event over fine-grained annotation  

% In the context of weak labels, existing research primarily focuses on how to effectively query or sample "positive" instances, or events that are present in the data. However, the significance of choosing informative "negative" samples—absent events—has received less attention. 

% The development of large-scale audio event detection has been hindered due to the lack of availability of annotated data. The 

% The development of large-scale audio event detection has been hindered for a long time by the availability of large labeled data. The problem lies in the annotation acquisition costs; for example, in the case of audio recording, one needs labeled sound events to 

% The machine learning approach of learning from weak labels has gained popularity in recent research [CITE] due to the following reasons: lower annotation costs, ease of scalabiility, training speed, and robustness to name a few. 



% While it is true that the space of the positive instances is few in the case of weak labels, the space of negative instances is large, and many of these negative instances will be largely irrelevant for the target class. Thus, it is imperative to choose the examples that we use to train the data, which is usually performed via the sampling strategy in the weak labels. We must determine better sampling strategies that can help select the negative samples that are most discriminative from the positive samples, and this case of the sample selection is well studied for strongly labeled data and underexplored for weak labels. 


% In the burgeoning landscape of machine learning, one of the most pressing challenges lies in the efficient and unbiased annotation of data for model training. Our work explores alternative sampling strategies that change how we handle negative instances in weak-label learning contexts.  Leveraging state-of-the-art active sampling techniques, our methodology targets the selection of negative bags based on their informativeness and diversity, thus allowing for a more balanced and effective training process. This work underscores a paradigm shift that substantially broadens the applicability of weak label learning across various domains including audio and image classification. We demonstrate that these sampling strategies not only outperform the standard random sampling in weak labels but also lead to gains in performance across diverse classes.  

% This is not merely an incremental advancement; it is a paradigm shift that substantially broadens the applicability of weak-label learning across various domains, including image and audio classification. As we will demonstrate, our approach not only outperforms existing methods but also offers an unparalleled blend of efficiency, accuracy, and robustness while operating within a reasonable labeling budget. 


% With effort saving and subjective bias suppression, scaling becomes a more efficient process as we can gather data quickly, especially when the data acquisition is easy nowadays while labeling is still far more labor-some.


% For a particular class in the weak-label classification task, we can define data bags into two categories: \textbf{\textit{Positive}} and \textbf{\textit{Negative}}. All data bags containing instances of this class, e.g., music, are considered positive or negative if there is no music sound.
% Here, the negative clips will consist of sounds from any other class, might become the dominating factor of our classifier's prediction, as they usually possess a much larger number than positive ones. A simple yet tricky question may arise: How do we choose the most informative negative bags for training a good weak classifier? To alleviate this situation, a negative selecting strategy comes as a rescue, where \textbf{\textit{Negative Sampling}} comes into place.

%As discussed above, we are interested in learning a good decision boundary between negative and positive bags with proper negative selection. To achieve this goal, we need to find an optimal sampling strategy to make better choices, telling that negative bags from classes are better or more informative for the current class' training. 



%On the contrary, negative sampling for weak label learning place more attention on the information of each negative bag itself. Furthermore, rather than rewriting the objective function, we can explicitly screen out the negative bags for each iteration's training.


% Many sampling strategies, which search for the most uncertain samples, have been proposed for active learning. For example, \cite{ghasemi2011active} proposed an uncertainty-based active learning algorithm for positive and unlabelled data. With the probability density of positive and unlabeled points estimated separately by Bayes rules, a margin-based and an Entropy-based approach are used to measure informativeness and to select the most uncertain samples for querying.
% To improve the quality of negative samples for tasks where there is high mutual information in the data, \cite{ma2020active} designed an active sampling strategy motivated by \cite{ash2019deep} to sample the most informative data for contrastive learning. It contains a gradient-based approach for uncertainty measurement, and \cite{ash2019deep}'s solution for samples' diversity. 
